FlexCast: genuine overlay-based atomic multicast

Atomic multicast is a communication abstraction where messages are propagated to groups of processes with reliability and order guarantees. Atomic multicast is at the core of strongly consistent storage and transactional systems. This paper presents FlexCast, the first genuine overlay-based atomic multicast protocol. Genuineness captures the essence of atomic multicast in that only the sender of a message and the message's destinations coordinate to order the message, leading to efficient protocols. Overlay-based protocols restrict how process groups can communicate. Limiting communication leads to simpler protocols and reduces the amount of information each process must keep about the rest of the system. FlexCast implements genuine atomic multicast using a complete DAG overlay. We experimentally evaluate FlexCast in a geographically distributed environment using gTPC-C, a variation of the TPC-C benchmark that takes into account geographical distribution and locality. We show that, by exploiting genuineness and workload locality, FlexCast outperforms well-established atomic multicast protocols without the inherent communication overhead of state-of-the-art non-genuine multicast protocols.

==> 3-background.tex <==
%!TEX root = 0-main.tex
\section{Background and motivation}
\label{sec:background}

%Several atomic multicast algorithms have been proposed in the literature.
In this section, we characterize atomic multicast protocols based on three aspects:
genuineness,
fault tolerance, and 
process communication.

\begin{figure*}[ht]
	\centering
    \includegraphics[width=1.2\columnwidth]{Figures/overlay.pdf}
    \caption{\small Three communication graphs used in atomic multicast algorithms involving groups $A, B, ..., E$: 
    (a)~a complete graph (the most common approach),
    (b)~a tree, and
    (c)~a complete directed acyclic graph or C-DAG (the approach used in this paper).
    In the graphs, directed edge $g \rightarrow h$ means that group $g$ can send messages to group $h$, and $h$ can receive messages from $g$ but not send messages to $g$.}
    %A tree is the minimal overlay for atomic multicast, and a complete DAG is the minimal overlay for genuine atomic multicast.}
    \label{fig:overlays}
\end{figure*}

\subsection{Genuine atomic multicast}
%\subsection{Genuine versus non-genuine atomic multicast}
\label{sec:genxngen}

Atomic multicast can be implemented by delegating the responsibility of ordering messages to a distinguished group of processes.
Every atomically multicast message $m$ is first sent to the distinguished group, which orders $m$ with respect to other multicast messages, and then propagates $m$ to its destination groups.
Although simple, this solution does not capture the spirit of atomic multicast.
%scale throughput (i.e., the number of messages ordered per time unit) with the number of groups, since eventually the distinguished group will become a performance bottleneck.

%In order to scale throughput with the number of groups, an 
%In this paper, we are interested in atomic multicast protocols that are ``genuine".
In a genuine atomic multicast protocol, only the sender and the destinations of a message coordinate to order the message. 
A genuine atomic multicast protocol does not depend on a fixed group of processes and does not involve processes unnecessarily. 
More precisely, a genuine atomic multicast algorithm should guarantee the following property \cite{GS01b}.

\begin{itemize}
    \item \emph{Minimality}: If a process $p$ sends or receives a message
    in run $R$, then some message $m$ is multicast in $R$, and $p$ is 
    $sender(m)$ or in a group in $m.dst$.
\end{itemize}


\subsection{Fault-tolerant atomic multicast}
\label{sec:ftxnft}

The first atomic multicast protocol is attributed to D. Skeen \cite{Birman}.
The protocol is genuine but does not tolerate failures.
%assumes that messages are multicast to a set of processes, not to a set of groups of processes.
A multicast message $m$ is first propagated to all its destinations.
Upon receiving the message, a destination assigns the message a local timestamp $lt$ and sends it to the other message destinations.
When a destination has received all $lt$s for the message, it computes the message's final timestamp $ft$ as the maximum among all of the message's local timestamps.
A message is only delivered after it has a $ft$ and messages are delivered in order of $ft$s.
%The protocol targets failure-free environments since the failure of a single process may block the execution.

Several fault-tolerant atomic multicast protocols are based on Skeen's ordering technique of exchanging timestamps (e.g., \cite{rodrigues1998scalatom,fritzke1998amcast,GS01b,FastCast17}).
In these fault-tolerant atomic multicast protocols, messages are addressed to sets of groups of processes, instead of a set of processes, as in the original Skeen protocol.
Although some processes in a group may fail, each group acts as a reliable entity, whose logic is replicated within the group using state machine replication \cite{Sch90}.
We assume a similar approach in the paper.

%\subsection{Fully versus partially connected communication graphs}
%\subsection{Complete communication graphs versus overlays}
\subsection{Overlay-based atomic multicast}
\label{sec:fullyxpartial}

Most atomic multicast protocols assume that processes can communicate directly with each other. 
In other words, the \emph{communication graph}, a directed graph where vertices represent groups of replicated server processes and an edge from group $g$ to group $h$ means that $g$ can send messages to $h$, is complete.
An alternative approach is to restrict communication by means of an overlay that determines how groups can communicate.
Restricting communication can lead to simpler atomic multicast algorithms, as in a tree overlay.
Moreover, if communication needs to be authenticated, as in Byzantine fault-tolerant protocols, a partially connected communication graph requires fewer keys to be maintained and exchanged between processes.
Finally, a complete communication graph is a reasonable assumption in systems that run within the same administrative domain (e.g., Google's Spanner [14]).
In other contexts, however (e.g., decentralized systems), multiple entities from different administrative domains collaborate but do not wish to establish connections with all other domains.
%it is unreasonable to expect that each process of one domain can communicate directly with all processes of another domain 
%(e.g., some processes in a domain may hide behind a firewall, instead of connecting directly to processes in other domains).

Figure~\ref{fig:overlays} shows three cases of interest.
All genuine atomic multicast algorithms we are aware of assume a complete communication graph (Figure~\ref{fig:overlays}~(a)).
A tree (Figure~\ref{fig:overlays}~(b)) is the minimum overlay needed by any atomic multicast protocol to support an arbitrary workload (i.e., messages can be multicast to any set of groups), as removing one edge from the overlay results in a partitioned graph.
ByzCast \cite{ByzCast} is an atomic multicast protocol that uses a tree overlay.
To order a message $m$, $m$ is first ordered within the lowest common ancestor group of groups in $m.dst$, in the worst case the root of the overlay tree. 
Then, $m$ is successively ordered by the lower groups in the tree until it reaches all groups in $m.dst$. 
ByzCast's main invariant is that lower groups in the tree preserve the order induced by higher groups.
Although simple, ByzCast is not genuine since a message may need to be ordered by a group that is not in the destination set of the message.
For example, in Figure~\ref{fig:overlays}~(b), a message multicast to groups $B$ and $C$ will first be ordered at $A$, and then propagated and ordered by  $B$ and $C$.


%\subsection{Genuine atomic multicast on overlays}
%%\subsection{Can overlay-based algorithms be genuine?}
%% falar do grafo dirigido full
%
%PROBABLY MOVE THIS TO SECTION IV
%We claim that a complete directed acyclic graph (C-DAG) is a necessary condition for genuineness in partially synchronous systems.
%To understand why, notice that in a C-DAG, each vertex has either an ongoing or outgoing edge with any other vertex.
%If there is no edge between groups $g$ and $h$ in the graph, then a message addressed to $g$ and $h$ needs to involve one or more groups not part of the message's destination, which violates minimality.\footnote{This observation assumes that to order a message addressed to two ore more groups, these groups need to communicate. It is easy to see that this holds in a partially synchronous system: }
%
%Similarly to a tree overlay, in a C-DAG a multicast message can be initially ordered at the lowest common ancestor (lca) group $g$ among the message's destinations and then be propagated by $g$ to the remaining destinations.
%In a C-DAG, however, the lca of a message can propagate the message directly to all remaining destinations of the message, respecting minimality.
%Differently from a tree overlay, in a C-DAG a group cannot deliver a message after it receives the message from its ancestor since groups can have more than one incoming edge and messages can arrive at a group from different ancestors.
%A group with multiple incoming edges must determine the correct order to deliver messages coming from its ancestors.
%
%For example, in Figure~\ref{fig:overlays}~(b), group $g_3$ can receive messages from $g_1$ and $g_2$.
%In an execution in which message $m_1$ is addressed to groups $g_1$, $g_2$ and $g_3$, and message $m_2$ is addressed to groups $g_2$ and $g_3$, group $g_3$ will receive $m_1$ from $g_1$ and $m_2$ from $g_2$.
%If $g_2$ delivers $m_2$ before $m_1$, then $g_3$ must respect this order, even if it may receive $m_1$ before $m_2$.
%Otherwise, $g_3$ would violate atomic multicast's acyclic order property.
%In the next section, we present a genuine algorithm that uses a C-DAG overlay and respects message interdependencies.





==> 5-evaluation_old.tex <==
%!TEX root = 0-main.tex

\section{Evaluation}
\label{sec:eval}

We implemented a \flexcast prototype, a Skeen's algorithm prototype, and a ByzCast prototype, all in Java.
In all cases, we consider single-process groups in order to evaluate the inherent costs of the protocols and avoid overhead introduced by replicating each group with state machine replication and Paxos.
Our experimental evaluation aims to compare the inherent latency costs of both protocols.
%, \elia{hence we deployed our prototypes in an emulated WAN, and we discuss latency improvements (and throughput evaluation as well), arguing about our findings.}

\subsection{Environment and deployment}

We now detail the environment where we performed the
evaluation of our prototypes.
The experimental setup was configured with 3 to 12 server machines and 12 client machines, all connected via a 1-Gbps switched network. 
The machines are equipped with Intel\textsuperscript{\textregistered} Xeon\textsuperscript{\textregistered} processor with 8 physical cores and 8 GB of RAM.
The software installed on the machines was Linux Ubuntu with kernel 4.15.0 (64 bits) and 64-bit Java virtual machine version 11.0.3. 

In our experiments, each group server connects to other servers via TCP, using the connection overlay according to the used protocol (i.e., complete graph for Skeen, a tree for ByzCast, and a C-DAG for \flexcast). {Since \flexcast is designed to optimize the latency perceived by the clients in a geographically distributed environment, we consider} an emulated wide-area network that resembles Amazon's EC2 cluster services (AWS). Each group in our experiments represents an AWS region and we experimented with 4 different deployments, varying the size of the system (i.e., number of groups/regions), where groups were distributed as depicted in Figure \ref{fig:regions}. The approximate latencies that we emulate among regions are based on \cite{awslatencies}.

\begin{figure}[ht]
    \includegraphics[width=1.06\columnwidth]{Figures/regions.pdf}
    \caption{\small AWS region distribution and gTPC-C deployments.}
    \label{fig:regions}
\end{figure}


% \begin{table*}[ht]
%     \tiny
%     \centering
%     \begin{tabular}{ |c|c|c|c|c|c|c|c|c|c|c|c|c| }
%      \hline
%      Regions / Latencies ($\pm$5ms) & ap-northeast-1 & ap-south-1 & ap-southeast-1 & ap-southeast-2 & ca-central-1 & eu-central-1 & eu-north-1 & eu-west-1 & eu-west-3 & sa-east-1 & us-east-1 & us-west-1 \\
%      \hline
%      ap-northeast-1 & 5 & 132 & 75 & 107 & 144 & 225 & 243 & 203 & 217 & 257 & 146 & 108  \\
%      ap-south-1 & 133 & 3 & 60 & 153 & 188 & 117 & 136 & 125 & 109 & 301 & 186 & 235  \\
%      ap-southeast-1 & 77 & 61 & 4 & 96 & 210 & 158 & 179 & 184 & 168 & 325 & 220 & 179  \\
%      ap-southeast-2 & 108 & 152 & 95 & 2 & 198 & 253 & 297 & 256 & 279 & 315 & 199 & 140 \\
%      ca-central-1 & 144 & 191 & 213 & 198 & 2 & 91 & 107 & 70 & 84 & 125 & 16 & 80 \\
%      eu-central-1 & 223 & 117 & 160 & 251 & 93 & 4 & 23 & 26 & 11 & 205 & 92 & 151 \\
%      eu-north-1 & 243 & 136 & 179 & 296 & 109 & 22 & 2 & 42 & 31 & 216 & 112 & 177 \\
%      eu-west-1 & 201 & 124 & 183 & 257 & 71 & 27 & 43 & 3 & 19 & 177 & 68 & 138 \\
%      eu-west-3 & 217 & 106 & 167 & 279 & 84 & 13 & 32 & 18 & 2 & 196 & 83 & 143  \\
%      sa-east-1 & 256 & 302 & 324 & 312 & 126 & 205 & 216 & 177 & 197 & 3 & 117 & 175  \\
%      us-east-1 & 146 & 191 & 219 & 200 & 17 & 92 & 111 & 68 & 83 & 115 & 5 & 62  \\
%      us-west-1 & 108 & 232 & 176 & 139 & 80 & 151 & 176 & 139 & 143 & 174 & 62 & 2 \\
%      \hline
%     \end{tabular}
%     \caption[]{Emulated latencies among AWS regions (in milliseconds, average values).}
%     \label{table:latencies}
% \end{table*}

In our setup, clients are uniformly distributed along regions and send requests to the nearest group. 
In our Skeen's algorithm implementation, upon receiving a request a group forwards the message to all other message destinations, all groups exchange timestamps, order and deliver the message according to these timestamps, and then reply to the client. 
In our ByzCast implementation, upon receiving a request the message's \lca forwards the message to its children that are either destination groups or ancestors of destination groups. Each intermediary group does the same. Each destination group replies to the client as soon as it delivers the message.
Similarly, in our \flexcast implementation, upon receiving a request the message's \lca forwards the message to all other message destinations and each group replies to the client as soon as it finishes the protocol and delivers the message. {Since we are interested in evaluating only communication costs (i.e., the multicast primitive) we do not implement any application logic, the messages carry an empty payload (no application data)}, hence there is no local execution cost.

% \subsection{Micro benchmarks}

\subsection{gTPC-C Benchmark}
\label{subsec:bench}

We implemented gTPC-C, a geographically distributed benchmark inspired by the well-established TPC-C benchmark \cite{tpcc}). 
We translate \tpcc warehouses into groups deployed in one or more AWS regions (see Figure~\ref{fig:regions}).
\tpcc transactions are multicast using FlexCast, ByzCast, or Skeen's algorithm to the warehouses/groups involved in a transaction. Clients operate in a closed loop issuing one transaction at a time (i.e., only send a new message after the previous message reply) and are co-located in the same region as their home warehouse. {Each experiment lasts for a period of approximately three minutes, in which clients collect and store latency data. 
We discard the first and last 10\% of the data collected during the experiment to avoid possibly noisy data during warm up and end of execution.} Clients can generate the following transactions, each with the given probability: new order (45\%), payment (43\%), order status (4\%), delivery (4\%), or stock level (4\%). The last three transactions are single-warehouse, that is, the message with the transaction is multicast only to the client's home warehouse. 
New order transactions can have from 5 to 15 items. Each item has a 2\% probability of being issued to a warehouse that is not the client's home warehouse, as defined by \tpcc. 
Payments can be multicast to at most two warehouses. 

To capture locality, when choosing an additional warehouse to the client's home warehouse, the client picks the nearest warehouse to its home warehouse with a configurable high probability {that we call \emph{locality rate}}; otherwise, the client chooses the next nearest warehouse, and so on, up to the farthest warehouse to the client's home warehouse.
For example, in a configuration with three groups, messages will most likely be addressed to groups either in America and Europe, or Europe and Asia. 
Only a few messages will involve groups in America and Asia or all three regions since such transactions would include items in the most distant warehouses.
Our criteria to define locality is inspired by a common wholesale supplier policy that when an item is not available in the nearest warehouse to a client (i.e., the home warehouse), it is shipped from the closest warehouse that has the item.
This locality specification implies that most messages are addressed to only two warehouses (same as in standard TPC-C), and some to three. Very few are addressed to more than three groups, therefore we don't consider these messages in our experiments.

%\flexcast performs better if the workload presents some sort of locality in message destinations, i.e. when messages are often addressed to groups close to each other. This is a very plausible assumption for many applications [source?]. Random destination workloads hurt \flexcast since messages addressed to distant groups in the DAG generate more intermediary communication steps due to acks and cascaded notification messages, needed to propagate dependencies.
%Therefore, we implement locality in the workload of messages issued by the clients, such that the destination set is generated with a configurable likelihood of involving groups geographically near to each other. 

\subsection{Results}

In the first set of experiments, we assess the performance of our protocol when compared to Skeen's algorithm, running the gTPC-C workload when deployed in a configuration with 6 warehouses/groups {and 95\% locality rate} (see Figure~\ref{fig:regions}).

\subsubsection{Throughput}

We conduct multiple experiments while gradually increasing the number of clients and measure the total number of transactions ordered by \flexcast and Skeen's algorithm.
Figure \ref{fig:tp} presents the results.
While \flexcast consistently outperforms Skeen's algorithm in all configurations considered, Skeen's algorithm scales better with the number of clients.
This effect can be seen by the slight bend of the throughput curve of \flexcast.

\begin{figure}[h]
	\centering
    \includegraphics[width=0.7\columnwidth]{evaluation/tp.pdf}
    \caption{\small \flexcast throughput vs. Skeen's when varying the number of clients.}
    \label{fig:tp}
\end{figure}

Table~\ref{tbl:scalfactor} compares the scalability of both protocols more systematically using a ``scalability factor", computed as the ratio between the  measured throughput of a given configuration and the ideal throughput of a fully scalable protocol. 
More precisely, if two consecutive configurations have $cf_i$ and $cf_j$ clients and measured throughput $mt_i$ and $mt_j$, respectively, then the scalability factor of the transition from $cf_i$ to $cf_j$ (i.e., $cf_i \rightarrow cf_j$) is computed as $mt_j / (mt_i * cf_i / cf_j )$.
Scalability factor of 1 is ideal, that is, a system that scales performance linearly with the number of clients.

In the experiments discussed next, we consider configurations with 192 clients. 
This is justified by the fact that neither \flexcast not Skeen's algorithm are under stress in this configuration, avoiding queuing effects that would interfere with their inherent latency.
Moreover, both protocols have similar scalability factor with 192 clients (i.e., $96 \rightarrow 192$ entry in Table~\ref{tbl:scalfactor}).

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|} \hline
				& Skeen's algorithm & ~~~~~\flexcast~~~~~ \\ \hline
$24 \rightarrow 48$ & 0.87 &	0.99 \\
$48 \rightarrow 96$ & 0.91 &	0.97 \\
$96 \rightarrow 192$ & 0.91 &	0.89 \\
$192 \rightarrow 360$ & 0.93 &	0.82 \\
$360 \rightarrow 480$ & 0.93 &	0.86 \\ \hline
\end{tabular}
\caption{Scalability factor.}
\label{tbl:scalfactor}
\end{table}%

\subsubsection{Latency}

In the next set of experiments we assess the latency perceived by the clients in deployments with different number of groups (i.e., TPC-C warehouses) distributed geographically. 
In Figure~\ref{fig:latgroups} we show the 95-th latency percentile (graph on the left) and latency Cumulative Distribution Function (CDF) for both \flexcast (middle) and Skeen (right) of gTPC-C in four different deployments with 3, 6, 9 and 12 groups {and 95\% locality rate}.

\begin{figure*}[t]
	\begin{subfigure}{0.685\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/lat.pdf}
		\caption{Latency 95-th percentile}
	\end{subfigure}
	\begin{subfigure}{0.685\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/cdf-flex.pdf}
		\caption{\flexcast latency CDF.}
	\end{subfigure}
	\begin{subfigure}{0.685\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/cdf-skeen.pdf}
		\caption{Skeen latency CDF.}
	\end{subfigure}
	\caption{Latency per number of groups.}
	\label{fig:latgroups}
\end{figure*}

Three aspects stand out in the results.
First, \flexcast consistently outperforms Skeen's algorithms, although the difference between the two protocols is more important with fewer groups.
{We attribute this result to the fact that, in a deployment with only three groups where each one is in a different macro-region with high latencies among them (e.g., group A in America, group B in Europe, and group C in Asia), \flexcast benefits more from two aspects that alleviate the cost of ordering messages in such a scenario: (i) while Skeen's protocol requires two communication steps involving groups A and B to order a message addressed to both of them, \flexcast will need only one communication step, that is, the lca (group A) forwarding the message to B; and (ii) the locality rate, since having a workload with a high locality rate increases the number of messages that \flexcast will be able to deliver using less communication steps than Skeen's algorithm. This gives \flexcast a large advantage since the cost for each communication step is high in geographical settings.}
Second, the latency of both protocols decreases with the increase in the number of groups.
This happens because as we introduce additional groups in a deployment, transactions that span multiple warehouses can use closer groups.
Third, \flexcast's latency is more stable than the latency of Skeen's protocol, as it can be seen from their latency CDFs.
For example, with three groups, 60\% of \flexcast messages experience a latency of approximately 200 milliseconds, while in Skeen's algorithm there is significant variation in the observed latency.


\begin{figure*}[t]
	\begin{subfigure}{0.685\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/lat6groups.pdf}
		\caption{Latency 95-th percentile.}
	\end{subfigure}
	\begin{subfigure}{0.685\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/cdf-flex-regions.pdf}
		\caption{\flexcast latency CDF.}
	\end{subfigure}
	\begin{subfigure}{0.685\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/cdf-skeen-regions.pdf}
		\caption{Skeen latency CDF.}
	\end{subfigure}
	\caption{Latency with 6 groups, per continent.}
	\label{fig:latcont}
\end{figure*}

{
In the next set of experiments, we consider latency per macro-regions (continents) of our distributed environment. The results presented in Figure \ref{fig:latcont} show that \flexcast's advantage mentioned in the previous paragraph also holds in deployments with more groups. In this case, we show a deployment with 6 groups where \flexcast shows much better performance than Skeen's algorithm also within each continent. 
Given \flexcast's C-DAG overlay and that each client in the gTPC-C benchmark is associated with the nearest warehouse, the locality rate in the workload makes the clients send most of their messages to their home warehouse and the next nearest warehouse. Therefore most messages in the system workload have a disjoint destination set. This increases \flexcast's advantage of having one less communication step than Skeen to order messages addressed to two groups when such groups are placed consecutively in the C-DAG. This result also shows that the locality rate, by imposing the behavior described above, also helps to decrease the number of auxiliary messages (\ack and \notif messages) needed to ensure consistency in the global total order, since interdependencies will be relatively fewer in such a scenario. 
}

\subsubsection{Locality}

{
As discussed in the previous sections, the locality rate is an important aspect that influences \flexcast's performance. We now evaluate the impact of varying the locality rate in a deployment with 6 groups.

\begin{figure}[htb]
	\centering
	\begin{subfigure}{0.7\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/latlocalities.pdf}
		\caption{Latency varying locality.}
		\label{fig:latlocality}
	\end{subfigure}
	\begin{subfigure}{0.7\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/tplocalities.pdf}
		\caption{Throughput varying locality.}
		\label{fig:tplocality}
	\end{subfigure}
	\caption{The impact of decreasing the locality rate in \flexcast performance compared to Skeen's.}
	\label{fig:locality}
\end{figure}

Figure \ref{fig:latlocality} shows the latency perceived by the clients (and Figure \ref{fig:tplocality} shows the average throughput) when decreasing the locality rate in the workload for both \flexcast and Skeen's algorithm. Figure \ref{fig:cdfslocality} shows the respective latency CDFs. Here we can see that lowering the locality rate from 95\% to 80\% decreases \flexcast's latency to the same level as Skeen's algorithm (although Skeen presents better throughput in this case). Decreasing the locality rate penalizes \flexcast since much more auxiliary messages will be needed to ensure consistency, as more interdependencies will be created in the system.
}

\begin{figure}[h]
	\centering
	\begin{subfigure}{0.7\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/cdf-flex-locality.pdf}
		\caption{\small \flexcast.}
	\end{subfigure}
	\begin{subfigure}{0.7\columnwidth}
		\includegraphics[width=\columnwidth]{evaluation/cdf-skeen-locality.pdf}
		\caption{\small Skeen.}
	\end{subfigure}
	\caption{The impact of decreasing the locality rate, latency CDFs.}
	\label{fig:cdfslocality}
\end{figure}

\subsubsection{Genuineness}

In the second and last set of experiments, we showcase the advantages of genuine protocols by comparing \flexcast to ByzCast in terms of latency perceived by the clients.
We compare the performance of \flexcast to different ByzCast overlay tree deployments, as depicted in Figure \ref{fig:treeoverlays}. We argue that these overlays can vary the ``degree'' of genuineness on ByzCast. Tree 1 allows for more genuine communication traffic, whereas trees 2 and 3 combine the aspects of the height of the tree and locality to worsen communication by making it less genuine and more remote.

\begin{figure*}[htb]
	\centering
	\begin{subfigure}{0.691\columnwidth}
		\includegraphics[width=\columnwidth]{Figures/TreeOverlays/Tree1.pdf}
		\caption{\small Tree 1.}
	\end{subfigure}
	\begin{subfigure}{0.691\columnwidth}
		\includegraphics[width=\columnwidth]{Figures/TreeOverlays/Tree2.pdf}
		\caption{\small Tree 2.}
	\end{subfigure}
	\begin{subfigure}{0.691\columnwidth}
		\includegraphics[width=\columnwidth]{Figures/TreeOverlays/Tree3.pdf}
		\caption{\small Tree 3.}
	\end{subfigure}
	\caption{ByzCast overlay tree deployments. The first tree allows for more genuineness, as messages addressed to groups in a sub-tree can enter the system in the sub-tree root group (lca of destinations). The second tree decreases genuineness as all messages need to involve the tree root group. The third three suffer the same problem as the second, but worse: the root group is the farthermost of many other groups.}
	\label{fig:treeoverlays}
\end{figure*}

Figure \ref{fig:vsbyzcast} presents the results .... EXPLICAR AQUI QUE ESPERAMOS A RESPOSTA DO PRIMEIRO NODE SOMENTE E ARGUMENTAR QUE SERVE PARA APLICACOES ONDE SERIALIZABILITY EH UM NIVEL DE CONSISTENCIA ACEITAVEL.

\begin{figure}[h]
	\centering
	\includegraphics[width=.7\columnwidth]{plots/vsByzCast/lat_nodes_1_2.pdf}
	\caption{Latency (90th percentile) in the first groups of destinations ($X$ axis) in \flexcast compared to ByzCast when varying the locality rate, and ``degree'' of genuineness.}
	\label{fig:vsbyzcast}
\end{figure}


==> 6-relwork.tex <==
%!TEX root = 0-main.tex

\section{Related Work}
\label{sec:rwork}

%\subsection{Atomic multicast protocols}
%\label{subsection:amcastAlgorithms}

In this section, we focus on atomic multicast protocols in which the order of messages results from agreement between the destination processes,
or destination-agreement protocols \cite{defago04total}.
%This class of protocols can be further classified in (i) timestamp-based, (ii) deterministic merge-based, and (iii) overlay-based protocols.

Among these, in timestamp-based protocols, processes first agree on the assignment of message timestamps and then deliver messages in timestamp order.
The discussed Skeen's algorithm \cite{Birman} is a seminal contribution to timestamp-based multicast protocols, however non fault-tolerant.
Several genuine protocols extend Skeen's timestamp technique to tolerate failures (e.g., \cite{fritzke1998amcast}, \cite{schiper2008inherent}, \cite{rodrigues1998scalatom}, \cite{FastCast17}, \cite{gotsman2019white}, \cite{Le2021RamCastRA}, \cite{Aguilera2019TheIO}).
Deterministic merge protocols (e.g., \cite{schiper2008inherent}, \cite{MPP2012}, \cite{marandi2010ring}, \cite{7371590}), are also destination-agreement as destination processes use a deterministic procedure to assure the delivery order, possibly violating genuineness.

In~\cite{DGF00}, a genuine atomic multicast protocol is proposed that imposes messages to
be relayed sequentially through their destination groups.  Groups are given a total order.
A multicast message $m$ is initially sent to the lowest group in $m.dst$ according to this order.
When the group receives $m$, it uses consensus to order and deliver $m$ inside the group, then $m$ is forwarded to the next group in $m.dst$, according to the total order of groups.
A group that delivers $m$ can only order the next message once it knows $m$ is ordered in all of 
$m.dst$,  which is after it receives an \textsc{end} message from the last group in $m.dst$.   
Although the dissemination of the message follows an order, the \textsc{end} message returns
to each group involved and therefore a fully connected topology is assumed. 
Besides needing $n+1$ steps to deliver a message, where $n$ is the number of destinations of 
the message, since groups remain locked until the \textsc{end} message arrives, this protocol
is affected by the convoy effect.

While the above algorithms assume full connectivity, there are also overlay-based algorithms. 
These rely on a predefined topology to propagate messages and to ensure atomic multicast properties.

As already discussed, Byzcast~\cite{ByzCast} is a byzantine fault-tolerant atomic multicast that arranges groups in a tree overlay.  A message $m$ enters the overlay in the lowest common ancestor of groups in $m.dst$.  A group that receives $m$ orders and then propagates $m$ down the tree, until all groups in $m.dst$ are reached.  Byzcast is not genuine: delivering a message addressed to multiple groups may involve intermediary groups not part of the destination set.    
This aspect has been further studied in this paper, Section \ref{subsec:overhead}.

The Arrow \cite{herlihy2006arrow} protocol is a non-fault tolerant overlay-based protocol that targets open groups.
It emerges from the combination of a reliable multicast protocol with a distributed swap protocol.
%
Arrow assumes a graph $G$ and a spanning tree $T$ on $G$.
Initially, each node $v$ in $T$ has $link(v)$ that is its neighbour in $T$ or
itself if $v$ is a sink (initially only the root of $T$).  
To multicast $m$ a node $v$ sends a message through $link(v)$, which
is forwarded to the root of the tree.   By definition,
the root has sent the last message before $m$.   As the message
is forwarded, edges change direction and $v$ becomes the new root
(that has sent the last message, which now is $m$).
Although genuine, this procedure may result in swap
messages traversing the diameter of $T$ and only then a multicast, using an
underlying reliable multicast, is issued.

==> correctness.tex <==

%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
%\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}

\section*{Appendix: Proof of correctness}

\begin{definition}  
{\it Message Order:} for any pair of messages $m \neq m'$, we say that $m < m'$ iff:
\begin{itemize}
    \item both $m$ and $m'$ are delivered at least by one same group, and $m$ is delivered before $m'$;
    \item or by transitivity:   $m < m'' \land m'' < m' \implies m < m'$.
\end{itemize}
\end{definition}

\vspace{2mm}
\begin{lemma}
    For any message $m$ atomically multicast to multiple groups, $m$ is received at all and only destination groups $d \in m.dst$.
    \label{lemma:LrcvMsg}
    \end{lemma}
    \vspace{1mm}
    {\sc Proof:} 
    By assumption \ref{ass:ingressMsg}, the client sends $m$ to $lca(m)$.   
    By assumption \ref{ass:topology}, any subset $m.dst$ of destinations is directly reached by $lca(m)$. 
    According to the algorithm, when $lca(m)$ receives $m$, it inconditionally $send$-$descendants(m)$ to all other destinations in $m.dst$ and only those.  
    As fault-tolerant groups and channels are supposed, eventually every destination group receives $m$ - and no other 
    group receives it.
    \hfill$\Box$

\vspace{2mm}
\begin{lemma}
    Let $m$ and $m'$ be messages such that $m.dst \cap m'.dst \neq \emptyset$.   
    There is a unique group that assigns a relative order to $m$ and $m'$, to be followed by all higher groups.
    \label{lemma:lcd}
\end{lemma}
    \vspace{1mm}
{\sc Proof:} 
    By assumption \ref{ass:ingressMsg}  $m$ and $m'$ ingress the overlay through their respective $lca$s
    and by lemma \ref{lemma:LrcvMsg} both  are received at their respective destinations.
    Since groups have a total order (assumption \ref{ass:topology}) 
    and $m.dst \cap m'.dst \neq \emptyset$, in the intersection there is a unique lowest group that 
    handles both $m$ and $m'$.  We call this group the lowest common destination of these messages, $lcd(m,m')$.
    Since message channels are directed towards higher groups only, the relative order of $m$ and $m'$ has 
    to be assigned at $lcd(m,m')$ and followed at higher groups, otherwise ordering could be violated.
    \hfill$\Box$
\vspace{2mm}


\begin{lemma}
    For any atomically multicast message $m$, the complete dependency information to deliver 
    $m$ is eventually received at each group in $m.dst$. 
    The {\it complete dependency information} to deliver $m$ at a group $g$ is the 
    information about any message $m'$ delivered before $m$, i.e.  $m' < m$ at each group lower than $g$. 
    \label{lemma:rcvDeps}
    \end{lemma}
    \vspace{1mm}
    {\sc Proof:} 
    By the algorithm:
    \begin{enumerate} 
        \item \label{lrcvDeps.fact-alg-1} each group $g$ keeps a history recording the order of messages it delivered and, for each message $m$ delivered, the previous messages $m'$ delivered at groups lower than $g$, such that $m'< m$;
        \item \label{rcvDeps.fact-alg-2} every message carries the history of the sending group, which enriches the history of each receiving group upon reception;
       % \item from Lemma \ref{lemma:LrcvMsg} each group in $m.dst$ receives $m$ from $lca(m)$;
        \item \label{rcvDeps.fact-alg-3} each group $g$ in $m.dst \setminus lca(m)$ sends ACKs to higher groups in $m.dst$;
        \item \label{rcvDeps.fact-alg-4} whenever any group $g$ in $m.dst$ has previously sent messages to a group $h$ lower than others in $m.dst$, $g$ sends NOTIFY to $h$.  Each notified group $h$ reacts sending ACKs to higher groups in $m.dst$ and inductively behaves as $g$ to NOTIFY further groups.  
        Since groups have a total order, this induction finishes.
    \end{enumerate} 

    From Lemma \ref{lemma:LrcvMsg} and facts above, it follows that each group in $m.dst$ is provided with the history of each lower group %in $m.dst$ as well as each other lower group 
that may be involved in messages ordered before $m$.
\hfill$\Box$
\vspace{2mm}

\begin{lemma}
    For any atomically multicast message $m$, any destination group in $m.dst$ 
    knows when the complete dependency information has been received.
    \label{lemma:completeDeps}
    \end{lemma}
    \vspace{1mm}
    {\sc Proof:} 
    By Lemma \ref{lemma:LrcvMsg} each group in $m.dst$ receievs $m$, by the algorithm
    it knows which are the lower groups in $m.dst$ and awaits for their respective ACKs.  
    Each ACK informs also if the sending group has notified
    other groups, from which by the algorithm further ACKs are awaited 
    (see Lemma \ref{lemma:rcvDeps}, facts \ref{rcvDeps.fact-alg-3} and \ref{rcvDeps.fact-alg-4}).   
    Thus, from the messages received, any destination of $m$ is able to detect if it has received 
    $ACK$s from all groups with messages ordered before $m$.
    \hfill$\Box$
    \vspace{2mm}

\begin{proposition}
(\textit{\flexcast is Genuine}) [ AQUI REVER A DEFINIÇÃO DE GENUÍNO ]
We say that a protocol is genuine if, given a run $R$, only processes that communicate in $R$ 
are involved in ordering messages in $R$. 
\end{proposition}

\vspace{2mm}
{\sc Proof:} 
From Lemma \ref{lemma:rcvDeps} it follows that 
all messages exchanged are restricted to processes that communicate in $R$.   \dots
\hfill$\Box$
\vspace{2mm}


\begin{proposition}
    (\textit{Validity and Agreement}) 
\end{proposition}
{\sc Proof:} 
Due to assumption \ref{ass:ft-groups}, Lemmas \ref{lemma:LrcvMsg}, \ref{lemma:rcvDeps} and \ref{lemma:completeDeps},
and by the algorithm, we have that all groups in $m.dst$ eventually have $m$ and are able to pass the evaluation of the first condition of {\bf can-deliver(m)}.   
%
It remains to check if there is any message $m'$ that should be deliverd before $m$.
If no $m'$ exists, then the group can deliver $m$.
%
If there exists such $m'$ it has to be first delivered.  
Assuming acyclic order, which is further discussed, the arguments above
and by induction on message dependecies, there will allways be
a message with no pending dependencies to deliver that will then 
enable further ones to be delivered, such that $m$ can be delivered.
Therefore, validity holds.
By the same arguments, agreement holds.
\hfill$\Box$
\vspace{2mm}

\begin{proposition}
    (\textit{Integrity}) 
\end{proposition}
{\sc Proof:} 
By Lemma \ref{lemma:LrcvMsg} a multicast message $m$ reaches all and only its destination groups.
Any other possible message (Acknowledgements or Notifications) do not convey messages
to be delivered.   So, a group $g$ delivers $m$ only if $g \in m.dst$ and $m$ has been multicast first.
\hfill$\Box$
\vspace{2mm}


\begin{proposition}
    (\textit{Prefix Order}) 
\end{proposition}
\vspace{2mm}
{\sc Proof:} 
    From Lemma \ref{lemma:lcd} there is a unique group, $lcd(m,m')$, that assigns the
    relative order among $m$ and $m'$.
    From Lemmas \ref{lemma:rcvDeps} and \ref{lemma:completeDeps} any further group in 
    $h \in m.\mathit{dst} \cap m'.\mathit{dst}$ receives and preserves 
    the order assigned by $lcd(m,m')$.   Thus prefix order holds.
\hfill$\Box$
\vspace{2mm}
    

\begin{proposition}
    (\textit{Acyclic Order}) 
\end{proposition}
\vspace{2mm}

To argue that \flexcast ensures acyclic order we use a contradiction.
Assume cycle $C$ exists: $m_1 < m_2 < \dotsc < m_k < m_1$.
Let $C$ be such that $m_k < m_1$ happens at group $h$ (i.e., $h$ delivers $m_k$ and then $m_1$), 
where  $h$ is the highest group in the overlay.
This is possible because the overlay induces a total order on groups.
%
We have to argue that before $h$ delivers $m_k$, it knows that $m_1$ precedes $m_k$, which leads to a contradiction since $h$ will not deliver $m_k$ before delivering $m_1$.

From the algorithm, we have the following:

\begin{itemize}

\item for each directly dependent pair $m < m'$, there is a $lcd(m,m')$ that delivers both messages - and decides their relative order;
\item any transitive dependency $m < m''$, by definition, comes from a concatenation of directly dependent pairs;
\item whenever a $lcd$  ...
\item whenever a message $m$ is received from ancestor $a$ by descendant $d$, 
         before delivering $m$, $d$ receives history information from any ancestor $a'$ descendant of $a$,
         if $a'$ is in $m.dst$ (Algo Strategies (a) and (b)) or 
         if $a'$ has any $m' < m$, directly or transitively (Algo Strategy (c));
\item ...
\end{itemize}

The proof of the claim is by induction on the size of cycle $C$.

\emph{Base step ($k=2$):} This is the case of $m_1 < m_2 <  m_1$.
In this case there is at least one group that delivers both messages involved. 
We have to assure that different groups that deliver both messages do not contradict.

Take $lcd(m_1, m_2)$ notice that, by definition,  
ancestors of $lcd(m_1, m_2)$ may handle one or other message, but not both.   
Considering no third message ($k=2$), $lcd(m_1, m_2)$ is free to assign a relative order to these.
W.l.g. assume $m_1 < m_2$.

By the algorithm, any descendant of $lcd(m_1, m_2)$ that is also a destination of 
$msg_i, i:\{1,2\}$ will receive either $[ \msg, m_i, history ]$ from $lcd$, if $lcd = lca(m_i)$,
or $[ \ack, m_i, history ]$, from $lcd$, if $lcd \neq lca(m_i)$.   In any case, any further
destination of both messages will receive $lcd$'s history.
Since, by the algorithm, a group only delivers a message when the complete information
arrived, upon delivery of $m_2$ in any descendant of $lcd(m_1, m_2)$ 
it is known that $m_1 < m_2$, contradicting the cycle assumption. 

\vspace{1mm}

\emph{Inductive step:} This is the case where $m_1 < m_2 < \dotsc < m_k < m_1$,
$h$ is the highest group and orders $m_k < m_1$.

As $h$ orders $m_k < m_1$, $h=lcd(m_k, m_1)$.
Since by the assumption there is $m_{k-1} < m_k$, 
then there is an ancestor of $h$, say $ah$, 
that ordered and delivered $m_{k-1} < m_k$, so $m_{k-1} < m_k$ is in $ah$'s history.
By the same arguments above, $m_k$ in $h$ is only delivered provided its history in 
ancestors of $h$ is known.  So $h$ knows that $m_{k-1} < m_k$ from $ah$.
By induction on the hypothesis, $ah$ knows the history of groups that delivered 
$m_{k-2} < m_{k-1}$ up to $m_{1}$, which is informed to $h$ with $m_k$ and 
thus $h$ knows that $m_1 < m_k$ before delivering $m_k$,
contradicting the cycle assumption. 


= = = = == = = = == = = = = = = = = = = = = = = = =
 
%\begin{proposition}
%    (\textit{Acyclic Order}) 
%\end{proposition}
%\vspace{2mm}
%
%To argue that \flexcast ensures acyclic order we use a contradiction.
%Assume cycle $C$ exists: $m_1 < m_2 < \dotsc < m_k < m_1$.
%Let $C$ be such that $m_k < m_1$ happens at group $h$ (i.e., $h$ delivers $m_k$ and then $m_1$), where  $h$ is the highest group in the overlay.
%This is possible because the overlay induces a total order on groups.
%
%Let $q$ be the $lcd$ group that delivers messages $m_1$ and $m_2$.   We consider all $lca$ combinatios for $m_1$ and $m_2$ (in Figure \ref{fig:causalpath2}, cases a, b, c and d).
%We claim that there is a causal path $P$ from the delivery of $m_2$ at $q$ to the reception of message $m_k$ at process $p$.
%%(which obviously implies that there is a path from m1 to mk) ???
%
%Since processes deliver messages following their causal dependencies, showing that causal path $P$ exists means that before $p$ delivers $m_k$, it knows that $m_1$ precedes $m_k$, which leads to a contradiction since $p$ will not deliver $m_k$ before delivering $m_1$.
%
%
%\vspace{2mm}
%
%The proof of the claim is by induction on the size of cycle $C$.
%
%\vspace{1mm}
%
%\emph{Base step ($k=2$):} This case corresponds to the four patterns involving messages $m_1$ and $m_2$ (see Figure \ref{fig:causalpath2}), having $r=p$. 
%For patterns (a) and (b), the claim follows directly.
%For patterns (c) and (d): Since $m_2$ is addressed to $q$ and $p$, and $p$ is below $q$ in the overlay, upon delivering $m_2$, accoording to the algorithm, $q$ sends an ACK message to $p$ (with all $q$'s dependencies) and thus there is a causal path.
%
%\vspace{1mm}
%
%\emph{Inductive step:}
%Assume there is a causal path between $m_2 < m_3 < \dotsc < m_k$. 
%We show that there is a causal message path from $m_1$ to $m_k$, 
%%possibly involving ACK messages,
%where $q$ delivers messages $m_1$ and $m_2$, and $r$ is one of the destinations of $m_2$ (together with $q$ and possibly other processes). 
%
%There are five possibilities for how $q$ creates a dependency between $m_1$ and $m_2$, and where $r$ is placed with respect to $q$ in the communication overlay (see Figure \ref{fig:causalpath2}).
%\begin{itemize}
%\item Cases (a) and (b). In these cases, $r$ is necessarily below $q$ in the overlay, since $q$ multicasts $m_2$ and otherwise $r$ would not be a destination of $m_2$. In these cases, $m_2$ multicast by $q$ to $r$ creates a causal path from $m_1$ to $m_2$ at $r$. 
%From the induction hypothesis, this leads to a causal path until $m_k$.
%
%\item Cases (c) and (d). In these cases, we consider that $r$ is below $q$ in the overlay. 
%Since both $q$ and $r$ are destinations of $m_2$ and $r$ is below $q$, from the algorithm, $q$ sends an ACK message to $r$ and $r$ waits for the ACK message before delivering $m_2$. 
%This creates a causal path between the delivery of $m_1$ and $m_2$ at $q$ and the delivery of $m_2$ at $r$. 
%From the induction hypothesis, it follows that there is a causal path all the way to the delivery of $m_k$ at $p$.
%
%\item Case (e). $r$  is positioned above $q$ in the communication overlay.  
%%
%Since there is a causal path $P$ between the delivery of $m_2$ at $r$ and the receive of $m_k$ at $p$, it is the case that $r$ sent a message in $P$, say $m_3$.
%Regarding  the generation of $m_3$, it could also be that $r = t$.
%Regarding the generation of $m_1$, it could be that  $s=q$.
%
%
%% When $r$ sends such message, say $m_3$, by the algorithm, if there are groups in $m_3.dst$ lower in the overlay than any group in $m_2.dst$ then, by the algorithm, $r$ sends a NOTIFY message to $q$ asking it to send an ACK messages those groups.   
%Since $r$ knows that it was involved in $m_2$ with $q$, below $r$ in the overlay, $r$ sends a NOTIFY message to $q$, and as a response, $q$ sends an ACK message in path $P$ to groups in $m_3.dst$ below $q$ (completing the information that $m_1$ is in the past of $m_3$).   Since groups can only deliver $m_3$ once these ACKs arrived, further messages after $m_3$ build a path $P$ to $m_k$ in $p$ starting from $m_2$ in $r$.
%%
%From the induction hypothesis that there is a path from $m_1$ to $m_k$.
%
%% \item Case (c.2) and (d.2). In these cases, $r$ is positioned above $q$ in the communication overlay. 
%% Since there is a causal path $P$ between the delivery of $m_2$ at $r$ and the receive of $m_k$ at $p$, it is the case that $r$ sent a message in $P$, say $m_3$.
%% % When $r$ sends such message, say $m_3$, by the algorithm, if there are groups in $m_3.dst$ lower in the overlay than any group in $m_2.dst$ then, by the algorithm, $r$ sends a NOTIFY message to $q$ asking it to send an ACK messages those groups.   
%% Since $r$ knows that it was involved in $m_2$ with $q$, below $r$ in the overlay, $r$ sends a NOTIFY message to $q$, and as a response, $q$ sends an ACK message in path $P$ to groups in $m_3.dst$ below $q$, completing the information that $m_1$ is in the past of $m_3$.   Since groups can only deliver $m_3$ once these ACKs arrived, further messages after $m_3$ build path $P$ starting from $r$.
%% It follows from this and the existence of a path from the induction hypothesis that there is a path from $m_1$ to $m_k$.
%\end{itemize}
%
%%\begin{figure}[ht]
%%	\centering
%%    \includegraphics[width=\columnwidth]{Figures/causal-paths-1.pdf}
%%    \caption{Causal paths 1}
%%    \label{fig:causalpath1}
%%\end{figure}
%
%\begin{figure}[ht]
%	\centering
%    \includegraphics[width=\columnwidth]{Figures/flexcastCases2.pdf}
%    \caption{Causal paths}
%    \label{fig:causalpath2}
%\end{figure}

\end{document}


